CoSe-Co: Text Conditioned Generative CommonSense Contextualizer

Pre-trained Language Models (PTLMs) have been shown to perform well on natural language tasks. Many prior works have leveraged structured commonsense present in the form of entities linked through labeled relations in Knowledge Graphs (KGs) to assist PTLMs. Retrieval approaches use KG as a separate static module which limits coverage since KGs contain finite knowledge. Generative methods train PTLMs on KG triples to improve the scale at which knowledge can be obtained. However, training on symbolic KG entities limits their applicability in tasks involving natural language text where they ignore overall context. To mitigate this, we propose a CommonSense Contextualizer (CoSe-Co) conditioned on sentences as input to make it generically usable in tasks for generating knowledge relevant to the overall context of input text. To train CoSe-Co, we propose a novel dataset comprising of sentence and commonsense knowledge pairs. The knowledge inferred by CoSe-Co is diverse and contain novel entities not present in the underlying KG. We augment generated knowledge in Multi-Choice QA and Open-ended CommonSense Reasoning tasks leading to improvements over current best methods on CSQA, ARC, QASC and OBQA datasets. We also demonstrate its applicability in improving performance of a baseline model for paraphrase generation task.

==> files/evaluation.tex <==
\section{Evaluation Results}

% %%% CSQA InHouse Split Results
% \begin{table}[h]
% \centering
% \scalebox{0.9}{
% \begin{tabular}{lcccc}
%     \toprule
%     \multicolumn{1}{c}{} & \multicolumn{1}{c}{20\%} & \multicolumn{1}{c}{60\%} & \multicolumn{2}{c}{100\%} \\
%     \multicolumn{1}{c}{\textbf{Methods}} & \textbf{IHtest} (\%) & \textbf{IHtest} (\%) & \textbf{IHdev} (\%) & \textbf{IHtest} (\%) \\
%     \midrule  
%     RoBERTa-large (w/o KG)  & 46.25~($\pm$0.63)  & 52.30~($\pm$0.16) & 73.07~($\pm$0.45) & 68.69 ($\pm$0.56) \\
%     \midrule
%     + {RGCN \scalebox{0.7}{\citep{schlichtkrull2018modeling}}} & 45.12~($\pm$0.69)  & 54.71~($\pm$0.37) & 72.69~($\pm$0.19) & 68.41~($\pm$0.66) \\
%     + {GconAttn \scalebox{0.7}{\citep{wang2019improving}}}  & 47.95~($\pm$0.11)  & 54.96~($\pm$0.69) & 72.61($~\pm$0.39) &
%     68.59~($\pm$0.96)\\
%     + {KagNet \scalebox{0.7}{\citep{kagnet}}}  & -- & -- & 73.47~($\pm$0.22) & 69.01~($\pm$0.76) \\
%     + {RN} \scalebox{0.7}{\citep{santoro2017simple}}  & 45.12~($\pm$0.69)  & 54.23~($\pm$0.28) & 74.57~($\pm$0.91) & 69.08~($\pm$0.21) \\
%     + {MHGRN} \scalebox{0.7}{\citep{feng-etal-2020-scalable}} & -- & -- & 74.45~($\pm$0.10)   & {71.11}~($\pm$0.81)  \\
%     + {PGQA} \scalebox{0.7}{\citep{pgqa}} & 58.25~($\pm$0.43)  & \underline{69.66}~($\pm$0.97) & \textbf{77.53}~($\pm$0.47)   & 71.19~($\pm$0.49)  \\
%     + {QA-GNN} \scalebox{0.7}{\citep{Yasunaga2021QAGNN}} & \underline{59.08}~($\pm$1.25)  & 68.70~($\pm$0.62) &  75.54~($\pm$0.42)   & \underline{72.29}~($\pm$0.43)  \\
%     \midrule
%     + \pgsname\ (\textbf{Ours}) & \textbf{61.20}~($\pm$0.19)  & \textbf{70.23}~($\pm$0.40) &  \underline{77.13}~($\pm$0.37)   & \textbf{72.87}~($\pm$0.31)  \\
%     \bottomrule 
% \end{tabular}
% }
% \vspace{-2mm}
% \caption{Performance comparison on varying proportions of \textbf{\textit{CommonsenseQA}} in-house split~\citep{kagnet}. As the official test is hidden, here we report the in-house dev (\textbf{IHdev}) and test (\textbf{IHtest}) accuracy, averaged across $5$ training runs. The numbers for a portion of baselines have been taken from \citet{pgqa} and \citet{Yasunaga2021QAGNN}, while others have been reproduced. The second-best number for each column is underlined.
% }
% % \vspace{-2mm}
% \label{tab:csqa_inhouse}
% \end{table}
% %%%

%%% OpenCSR Zero-Shot Results
% \begin{table}[h]
% \centering
% \scalebox{1.0}{
% \begin{tabular}{lcllll}
% \hline
%                                              & \textbf{Metric}               & \multicolumn{4}{c}{\textbf{K}} \\ \hline
%                                              & \multicolumn{1}{l}{} & 10      & 20     & 30     & 40     \\ \cline{3-6} 
% \multicolumn{1}{c}{\multirow{2}{*}{\textbf{DrFact}}} & Hits@K               & 0.35    & 0.49   & 0.55   & 0.60   \\
% \multicolumn{1}{c}{}                         & Recall@K             & 0.12    & 0.19   & 0.22   & 0.25   \\ \hline
% \multirow{2}{*}{(\textbf{Ours})}                        & Hits@K               & 0.27    & 0.42   & 0.46   & 0.51   \\
%                                              & Recall@K             & 0.09    & 0.14   & 0.17   & 0.19   \\ \hline
% \end{tabular}}
% \caption{Performance comparison on \textbf{OpenCSR dataset, ARC}~\citep{lin-etal-2021-differentiable}. As the official test is hidden, here we report numbers on the validation split.
% }
% \label{tab:opencsr_eval}
% \end{table}
%%%

%%% OpenCSR Results
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\scalebox{0.85}{
\begin{tabular}{ll|ccc|ccc|ccc}
\hline
\multicolumn{1}{l}{} &
   &
  \multicolumn{3}{c|}{ARC} &
  \multicolumn{3}{c|}{QASC} &
  \multicolumn{3}{c}{OBQA} \\ \hline
\multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Hits@K}} &
  \cellcolor[HTML]{EFEFEF}{H@10} &
  \cellcolor[HTML]{EFEFEF}{H@30} &
  \cellcolor[HTML]{EFEFEF}{H@50} &
  \cellcolor[HTML]{EFEFEF}{H@10} &
  \cellcolor[HTML]{EFEFEF}{H@30} &
  \cellcolor[HTML]{EFEFEF}{H@50} &
  \cellcolor[HTML]{EFEFEF}{H@10} &
  \cellcolor[HTML]{EFEFEF}{H@30} &
  \cellcolor[HTML]{EFEFEF}{H@50} \\ \hline
\multicolumn{2}{l|}{{DrFact \scalebox{0.7}{\citep{lin-etal-2021-differentiable}}}} &
  {\color[HTML]{000000} 36.09} &
  {\color[HTML]{000000} 53.25} &
  {\color[HTML]{000000} 64.50} &
  {\color[HTML]{000000} 21.78} &
  {\color[HTML]{000000} 37.62} &
  {\color[HTML]{000000} 51.49} &
  {\color[HTML]{000000} 6.12} &
  {\color[HTML]{000000} 11.85} &
  {\color[HTML]{000000} 16.51} \\
\multicolumn{2}{l|}{{T5-base \scalebox{0.7}{\citep{raffel2019t5}}}} &
  {\color[HTML]{000000} 49.70} &
  {\color[HTML]{000000} 67.46} &
  {\color[HTML]{000000} 71.01} &
  {\color[HTML]{000000} 33.66} &
  {\color[HTML]{000000} 47.52} &
  {\color[HTML]{000000} 53.47} &
  {\color[HTML]{000000} 17.42} &
  {\color[HTML]{000000} 29.55} &
  {\color[HTML]{000000} 37.88} \\
\multicolumn{2}{l|}{+ {Paths from \pgsname}} &
  {\color[HTML]{000000} \textbf{50.89}} &
  {\color[HTML]{000000} 63.91} &
  {\color[HTML]{000000} 69.23} &
  {\color[HTML]{000000} 30.69} &
  {\color[HTML]{000000} 47.52} &
  {\color[HTML]{000000} 56.44} &
  {\color[HTML]{000000} 20.45} &
  {\color[HTML]{000000} 34.09} &
  {\color[HTML]{000000} \textbf{45.45}} \\
\multicolumn{2}{l|}{+ {Concepts from \pgsname}} &
  {\color[HTML]{000000} 44.97} &
  {\color[HTML]{000000} \textbf{66.86}} &
  {\color[HTML]{000000} \textbf{73.37}} &
  {\color[HTML]{000000} \textbf{35.64}} &
  {\color[HTML]{000000} \textbf{47.52}} &
  {\color[HTML]{000000} \textbf{57.43}} &
  {\color[HTML]{000000} \textbf{21.21}} &
  {\color[HTML]{000000} \textbf{35.61}} &
  {\color[HTML]{000000} 42.42} \\ \hline
\multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{Recall@K}} &
  \cellcolor[HTML]{EFEFEF}{R@10} &
  \cellcolor[HTML]{EFEFEF}{R@30} &
  \cellcolor[HTML]{EFEFEF}{R@50} &
  \cellcolor[HTML]{EFEFEF}{R@10} &
  \cellcolor[HTML]{EFEFEF}{R@30} &
  \cellcolor[HTML]{EFEFEF}{R@50} &
  \cellcolor[HTML]{EFEFEF}{R@10} &
  \cellcolor[HTML]{EFEFEF}{R@30} &
  \cellcolor[HTML]{EFEFEF}{R@50} \\ \hline
\multicolumn{2}{l|}{{DrFact \scalebox{0.7}{\citep{lin-etal-2021-differentiable}}}} &
  {\color[HTML]{000000} 12.60} &
  \multicolumn{1}{c}{{\color[HTML]{000000} 21.05}} &
  {\color[HTML]{000000} 27.27} &
  {\color[HTML]{000000} 12.38} &
  {\color[HTML]{000000} 22.28} &
  {\color[HTML]{000000} 29.70} &
  {\color[HTML]{000000} 6.12} &
  {\color[HTML]{000000} 11.85} &
  {\color[HTML]{000000} 16.51} \\
\multicolumn{2}{l|}{{T5-base \scalebox{0.7}{\citep{raffel2019t5}}}} &
  {\color[HTML]{000000} 15.98} &
  \multicolumn{1}{c}{{\color[HTML]{000000} 28.30}} &
  {\color[HTML]{000000} 33.93} &
  {\color[HTML]{000000} 18.98} &
  {\color[HTML]{000000} 26.40} &
  {\color[HTML]{000000} 30.53} &
  {\color[HTML]{000000} 8.52} &
  {\color[HTML]{000000} 14.61} &
  {\color[HTML]{000000} 18.71} \\
\multicolumn{2}{l|}{+ {Paths from \pgsname}} &
  {\color[HTML]{000000} \textbf{16.87}} &
  \multicolumn{1}{c}{{\color[HTML]{000000} 27.45}} &
  {\color[HTML]{000000} 33.73} &
  {\color[HTML]{000000} 17.49} &
  {\color[HTML]{000000} 28.05} &
  {\color[HTML]{000000} \textbf{33.33}} &
  {\color[HTML]{000000} 9.90} &
  {\color[HTML]{000000} 16.53} &
  {\color[HTML]{000000} \textbf{22.42}} \\
\multicolumn{2}{l|}{+ {Concepts from \pgsname}} &
  {\color[HTML]{000000} 15.12} &
  \multicolumn{1}{c}{{\color[HTML]{000000} \textbf{28.99}}} &
  {\color[HTML]{000000} \textbf{35.21}} &
  {\color[HTML]{000000} \textbf{19.64}} &
  {\color[HTML]{000000} \textbf{28.05}} &
  {\color[HTML]{000000} 33.00} &
  {\color[HTML]{000000} \textbf{9.96}} &
  {\color[HTML]{000000} \textbf{17.35}} &
  {\color[HTML]{000000} 21.10} \\ \hline
\end{tabular}}
\caption{Performance comparison on the $3$ \textbf{OpenCSR} datasets~\citep{lin-etal-2021-differentiable}. As the official test is hidden, here we report numbers on the validation split.
}
\label{tab:opencsr_eval}
\end{table}
%%%

% % Please add the following required packages to your document preamble:
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table}[t]
% \centering
% \scalebox{0.85}{
% \begin{tabular}{cl|crc|crc|crc}
% \hline
% \multicolumn{1}{l}{} &
%   &
%   \multicolumn{3}{c|}{\cellcolor[HTML]{C9DAF8}ARC} &
%   \multicolumn{3}{c|}{\cellcolor[HTML]{D9D2E9}QASC} &
%   \multicolumn{3}{c}{\cellcolor[HTML]{FCE5CD}OBQA} \\ \hline
% \multicolumn{2}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{Hits@K}} &
%   H@10 &
%   H@30 &
%   H@50 &
%   H@10 &
%   H@30 &
%   H@50 &
%   H@10 &
%   H@30 &
%   H@50 \\ \hline
% \multicolumn{2}{c|}{DrFact} &
%   \cellcolor[HTML]{ECF2FD}36.09 &
%   \cellcolor[HTML]{E3ECFC}53.25 &
%   \cellcolor[HTML]{DDE8FB}64.50 &
%   \cellcolor[HTML]{F7F6FB}21.78 &
%   \cellcolor[HTML]{F1EFF7}37.62 &
%   \cellcolor[HTML]{ECE8F4}51.49 &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} \\
% \multicolumn{2}{c|}{T5 (Wihout Paths)} &
%   \cellcolor[HTML]{E5EDFC}49.70 &
%   \cellcolor[HTML]{DBE7FB}67.46 &
%   \cellcolor[HTML]{D9E5FB}71.01 &
%   \cellcolor[HTML]{F3F0F8}33.66 &
%   \cellcolor[HTML]{EDEAF5}47.52 &
%   \cellcolor[HTML]{EBE7F4}53.47 &
%   \cellcolor[HTML]{FFFBF7}17.42 &
%   \cellcolor[HTML]{FFF8F1}29.55 &
%   \cellcolor[HTML]{FEF6ED}37.88 \\
% \multicolumn{2}{c|}{Ours (Paths with T5)} &
%   \cellcolor[HTML]{E4EDFC}\textbf{50.89} &
%   \cellcolor[HTML]{DDE8FB}63.91 &
%   \cellcolor[HTML]{DAE6FB}69.23 &
%   \cellcolor[HTML]{F7F6FB}21.78 &
%   \cellcolor[HTML]{F1EFF7}37.62 &
%   \cellcolor[HTML]{ECE8F4}51.49 &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} \\
% \multicolumn{2}{c|}{Ours (Paths as Concepts)} &
%   \cellcolor[HTML]{E7EFFC}44.97 &
%   \cellcolor[HTML]{DBE7FB}\textbf{66.86} &
%   \cellcolor[HTML]{D8E4FA}\textbf{73.37} &
%   \cellcolor[HTML]{F2EFF8}\textbf{35.64} &
%   \cellcolor[HTML]{EDEAF5}\textbf{47.52} &
%   \cellcolor[HTML]{EAE6F3}\textbf{57.43} &
%   \cellcolor[HTML]{FFFAF5}\textbf{21.21} &
%   \cellcolor[HTML]{FEF6EE}\textbf{35.61} &
%   \cellcolor[HTML]{FEF4EA}\textbf{42.42} \\ \hline
% \multicolumn{2}{c|}{\cellcolor[HTML]{D9D9D9}\textbf{Recall@K}} &
%   R@10 &
%   R@30 &
%   R@50 &
%   R@10 &
%   R@30 &
%   R@50 &
%   R@10 &
%   R@30 &
%   R@50 \\ \hline
% \multicolumn{2}{c|}{DrFact} &
%   \cellcolor[HTML]{F9FBFF}12.60 &
%   \multicolumn{1}{c}{\cellcolor[HTML]{F4F8FE}21.05} &
%   \cellcolor[HTML]{F1F5FE}27.27 &
%   \cellcolor[HTML]{FBFAFD}12.38 &
%   \cellcolor[HTML]{F7F5FB}22.28 &
%   \cellcolor[HTML]{F4F2F9}29.70 &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} \\
% \multicolumn{2}{c|}{T5 (Wihout Paths)} &
%   \cellcolor[HTML]{F7FAFE}15.98 &
%   \multicolumn{1}{c}{\cellcolor[HTML]{F0F5FE}28.30} &
%   \cellcolor[HTML]{EDF3FD}33.93 &
%   \cellcolor[HTML]{F8F7FB}18.98 &
%   \cellcolor[HTML]{F5F4FA}26.40 &
%   \cellcolor[HTML]{F4F2F9}30.53 &
%   \cellcolor[HTML]{FFFDFB}8.52 &
%   \cellcolor[HTML]{FFFCF8}14.61 &
%   \cellcolor[HTML]{FFFBF6}18.71 \\
% \multicolumn{2}{c|}{Ours (Paths withT5)} &
%   \cellcolor[HTML]{F6F9FE}\textbf{16.87} &
%   \multicolumn{1}{c}{\cellcolor[HTML]{F1F5FE}27.45} &
%   \cellcolor[HTML]{EDF3FD}33.73 &
%   \cellcolor[HTML]{FBFAFD}12.38 &
%   \cellcolor[HTML]{F7F5FB}22.28 &
%   \cellcolor[HTML]{F4F2F9}29.70 &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{1}{l}{} \\
% \multicolumn{2}{c|}{Ours (Paths as Concepts)} &
%   \cellcolor[HTML]{F7FAFE}15.12 &
%   \multicolumn{1}{c}{\cellcolor[HTML]{F0F5FD}\textbf{28.99}} &
%   \cellcolor[HTML]{ECF2FD}\textbf{35.21} &
%   \cellcolor[HTML]{F8F7FB}\textbf{19.64} &
%   \cellcolor[HTML]{F5F3F9}\textbf{28.05} &
%   \cellcolor[HTML]{F3F1F8}\textbf{33.00} &
%   \cellcolor[HTML]{FFFDFB}\textbf{9.96} &
%   \cellcolor[HTML]{FFFBF7}\textbf{17.35} &
%   \cellcolor[HTML]{FFFAF5}\textbf{21.10} \\ \hline
% \end{tabular}}
% \caption{Performance comparison on the $3$ \textbf{OpenCSR} datasets~\citep{lin-etal-2021-differentiable}. As the official test is hidden, here we report numbers on the validation split.
% }
% \label{tab:opencsr_eval}
% \end{table}

% \noindent \textbf{CSQA}{  } We use the approach described in Section \ref{sec:down_csqa} with RoBERTa-base~\citep{roberta} as the contextual encoder. Table \ref{tab:csqa_inhouse} shows the corresponding results on the commonsense question-answering benchmark. We observe that our approach outperforms all comparable methods, including QA-GNN~\citep{Yasunaga2021QAGNN} that uses an entire static KG on the fly. PGQA~\citep{pgqa} is the most similar to our approach and primarily differs on how the commonsense paths are obtained; we observe a significant gain over them, signifying the relevance and applicability of inferences generated by \pgsname.\\

% \noindent \textbf{OpenCSR}{  } Table \ref{tab:opencsr_eval} presents the comparison between the dataset-specific state-of-the-art approach for OpenCSR, DrFact~\citep{lin-etal-2021-differentiable}, and the zero-shot adaptation of \pgsname\ for the same dataset. We observe that even with this large evident difference between the state of the two systems, our zero-shot approach is able to perform on-par with DrFact on both measures of Hits\@K and Recall\@K. We remain in close vicinity of their performance, with the minimum difference going as low as 7\%, for K=20.

% \begin{itemize}
%     \item \textbf{CSQA}
%     \begin{itemize}
%         \item[--] Better than state-of-the-art while being generalizable and task-agnostic
%     \end{itemize}
%     \item \textbf{OpenCSR}
%     \begin{itemize}
%         \item[--] Close to state-of-the-art even when evaluated in a zero-shot setting
%         \item[--] Consistent across variable K
%     \end{itemize}
% \end{itemize}
